Revisiting LLMs as Zero-Shot Time-Series Forecasters: Small Noise Can Break Large Models

Large Language Models (LLMs) have shown remarkable performance across diverse tasks without domain-specific training, fueling interest in their potential for time-series forecasting. While LLMs have shown potential in zero-shot forecasting through prompting alone, recent studies suggest that LLMs lack inherent effectiveness in forecasting. Given these conflicting findings, a rigorous validation is essential for drawing reliable conclusions. In this paper, we evaluate the effectiveness of LLMs as zero-shot forecasters compared to state-of-the-art domain-specific models. Our experiments show that LLM-based zero-shot forecasters often struggle to achieve high accuracy due to their sensitivity to noise, underperforming even simple domain-specific models. We have explored solutions to reduce LLMs' sensitivity to noise in the zero-shot setting, but improving their robustness remains a significant challenge. Our findings suggest that rather than emphasizing zero-shot forecasting, a more promising direction would be to focus on fine-tuning LLMs to better process numerical sequences. Our experimental code is available at https://github.com/junwoopark92/revisiting-LLMs-zeroshot-forecaster.

==> Figures/desc_QA_prompt.tex <==
\begin{figure}[h!]
    \centering
    \begin{minipage}{0.42\textwidth}
        \fbox{
            \begin{minipage}{\textwidth}
                \fontsize{10}{10}\selectfont
                \textbf{(a) Sequence Predidction} \\
                \rule{\textwidth}{0.4pt}
                \fontsize{7}{8}\selectfont                
                This is the description of the time series you are predicting. Understanding it will help with your prediction:\\ 
                \{Context\} \\

                You are tasked with predicting the next 5 data points based on the given observed sequence consisting of 20 data points. \\

                Please predict next sequence following input sequence without producing any additional text. Do not say anything like 'the next terms in the sequence are', just return the numbers. Input Sequence: -12, -13, -15, -7, -11, -6, 43, 98, 43, -10, -11, -9, -11, -12, -9, -10, -12, -8, -9, -13, 
                \rule{\textwidth}{0.4pt}
                \fontsize{7}{8}\selectfont
                \textbf{Response}: -9, -10, -12, -8, -9
            \end{minipage}
        }
    \vspace{3mm}
    \end{minipage}
    \begin{minipage}{0.42\textwidth}
        \fbox{
            \begin{minipage}{\textwidth}
                \fontsize{10}{10}\selectfont
                \textbf{(b) Sequence Prediction with QA} \\
                \rule{\textwidth}{0.4pt}
                \fontsize{7}{8}\selectfont
                
                This is the description of the time series you are predicting. Understanding it will help with your prediction:\\ 
                \{Context\} \\

                You are tasked with predicting the next 5 data points based on the given observed sequence consisting of 20 data points. \\
                Let's think step by step. \\

                \textbf{Step 1)} What is the expected value of the peak occurring in the forecast period? Answer with one number.\\

                \textbf{Step 2)} What is the position of the peak occurring in the forecast period? The position starts from 0. Answer with one number. \\
                
                \textbf{Step 3)} Considering the answers to previous steps, please predict next sequence following input sequence without producing any additional text. Do not say anything like 'the next terms in the sequence are', just return the numbers. Input Sequence: -12, -13, -15, -7, -11, -6, 43, 98, 43, -10, -11, -9, -11, -12, -9, -10, -12, -8, -9, -13, 
               \rule{\textwidth}{0.4pt}
                \fontsize{7}{8}\selectfont
                \textbf{Response}: \\ 
                \textbf{Answer 1)}  196 \\
                \textbf{Answer 2)}  2 \\
                \textbf{Answer 3)} -9, -10, -12, -8, -9

            \end{minipage}
        }
    \end{minipage}

    \caption{Examples of self-correcting in our annotation process: (a) key country extraction and (b) relationship labeling. In (a), the initial list included `CHN' and `RUS' incorrectly. `CHN' was mentioned only as a sea name, and `RUS' was related to unclear facts. Through self-correcting including verification and explanation, they were removed. In (b), the initial relationship prediction followed the negative tone of the article. The self-correcting process adjusted it to a neutral score, aligning with domain expert opinions.}
    \label{main-fig:correcting-samples}
\end{figure}

==> Figures/desc_two_scenarios_with_context.tex <==
\begin{figure}[h!]
\begin{center}
  \includegraphics[width=1.0\linewidth]{Figures/figures/acl25_data_desc.pdf}
\end{center}
\caption{Example of the relative selection strategy in our AutoCon.}
\label{fig:increasing-noise}
\end{figure}

==> Tables/exp_peak_qa_format.tex <==
\begin{table}[]
\centering
 % 테이블 사이 간격 조정
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l|l|ccc@{}}
\toprule
\textbf{Model (Tasks)}                        & \textbf{Answer Format} & \multicolumn{1}{c}{\textbf{Making Peak}} & \multicolumn{1}{c}{\textbf{Height \& Pos}} & \multicolumn{1}{l}{\textbf{Seq. MAE}} \\ \midrule
GPT-4o (Seq. Prediction)                      & Seq.                   & 0.9800                                   & 0.3467                                     & \multicolumn{1}{r}{\textbf{1.5046}}            \\ \midrule
GPT-4o (QA)                                   & Short Answer           & \textbf{1.0000}                          & \textbf{1.0000}                            & -                                     \\ \midrule
\multirow{2}{*}{GPT-4o (QA, Seq. Prediction)} & Short Answer           & 1.0000                                   & 0.9933                                     & -                                     \\
                                              & Seq.                   & 0.9733                                   & 0.6800                                     & \multicolumn{1}{r}{1.6246}            \\ \bottomrule 
\end{tabular}
}

\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\end{table}

==> Tables/exp_trend_qa_format.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l|l|ccc@{}}
\toprule
\textbf{Model (Tasks)}                        & \textbf{Answer Format} & \multicolumn{1}{c}{\textbf{Making Shift}} & \multicolumn{1}{c}{\textbf{\quad Slope \quad\quad}} & \multicolumn{1}{l}{\textbf{Seq. MAE}} \\ \midrule
GPT-4o (Seq. Prediction)                      & Seq.                   & 0.9833                                   & 0.5867                                     & \multicolumn{1}{r}{\textbf{0.2640}}            \\ \midrule
GPT-4o (QA)                                   & Short Answer           & \textbf{1.0000}                          & \textbf{0.9400}                            & -                                     \\ \midrule
\multirow{2}{*}{GPT-4o (QA, Seq. Prediction)} & Short Answer           & 1.0000                                   & 0.9200                                     & -                                     \\
                                              & Seq.                   & 0.9400                                   & 0.8467                                     & \multicolumn{1}{r}{0.2644}            \\ \bottomrule 
\end{tabular}
}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\end{table}

==> Tables/proposal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{c|l|rrr}
\toprule
\textbf{Method}                                                             & \multicolumn{1}{c|}{\textbf{LLM}} & \multicolumn{1}{c}{\textbf{Prec.}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F1}} \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}AnomLLM\\ (Text)\end{tabular}}   & Gemini-1.5-Flash                       & 2.01                               & 2.47                                & 1.89                            \\
                                                                            & GPT-4o-Mini                            & 12.16                              & 12.60                               & 12.04                           \\
                                                                            & GPT-4o                                 & 19.69                              & 17.61                               & 17.75                           \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}AnomLLM\\ (Vision)\end{tabular}} & Gemini-1.5-Flash                       & 39.60                              & 59.62                               & 43.56                           \\
& GPT-4o-Mini                            & 35.91                              &  38.60                              & 36.24                           \\
                                                                            & GPT-4o                                 & 39.53                              & 50.59                               & 42.03                           \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Our \\ (Text)\end{tabular}}      & GPT-4o-Mini                            & 37.13                              & 49.47                               & 39.39                           \\
                                                                            & GPT-4o                                 & \textbf{51.64}                     & \textbf{70.22}                      & \textbf{55.49}                  \\ \bottomrule
\end{tabular}
\end{table}
